NirvaWave: An Accurate and Efficient Near Field Wave Propagation Simulator for 6G and Beyond

The extended near-field range in future mm-Wave and sub-THz wireless networks demands a precise and efficient near-field channel simulator for understanding and optimizing wireless communications in this less-explored regime. This paper presents NirvaWave, a novel near-field channel simulator, built on scalar diffraction theory and Fourier principles, to provide precise wave propagation response in complex wireless mediums under custom user-defined transmitted EM signals. NirvaWave offers an interface for investigating novel near-field wavefronts, e.g., Airy beams, Bessel beams, and the interaction of mmWave and sub-THz signals with obstructions, reflectors, and scatterers. The simulation run-time in NirvaWave is orders of magnitude lower than its EM software counterparts that directly solve Maxwell Equations. Hence, NirvaWave enables a user-friendly interface for large-scale channel simulations required for developing new model-driven and data-driven techniques. We evaluated the performance of NirvaWave through direct comparison with EM simulation software. Finally, we have open-sourced the core codebase of NirvaWave in our GitHub repository (https://github.com/vahidyazdnian1378/NirvaWave).

==> comments.tex <==
%Scalar diffraction theory\cite{} models the EM waves as complex scalar quantities that only contain magnitude information, unlike traditional modeling where EM waves are considered to have both magnitude and direction. This theory can serve as the basic principle for accurate near-field channel modeling. Particularly, in \acrshort{design} we use Rayleigh-Sommerfeld integral theory, which is a scalar wave approximation method, to model the near-field propagation of EM waves. According to this theory, each point on the source plane is assumed to radiate spherical waves along the transverse direction based on the Huygens-Fresnel principle \cite{}.  The Rayleigh-Sommerfeld integral computes the resultant electric field by aggregating the contributions from each source point to the desired location. 


% In general, scenarios where there are arbitrary numbers of reflectors and blockages in the environment, we need to first transform the objects' properties from the original coordinate systems to corresponding information in the coordinate system of the reflector plane from which we intend to find the reflected EM wave propagation. hence we should define the coordinate transformation matrix $\mathcal{R}_r$ and transformed object orientation angle $\theta^*$. 
% \begin{equation}
%     \begin{aligned}
%         &\left[O^*_x,O^*_y\right] = \mathcal{R}_r \times  (\left[O_{R_x},O_{R_y}\right]-\left[O_x,O_y\right]) \\[0.5em]
%         &\mathcal{R}_r = \begin{bmatrix}
%         \cos(\theta_{ref}+\pi/2) & -\sin(\theta_{ref}+\pi/2)\\
%         \sin(\theta_{ref}+\pi/2)& \cos(\theta_{ref}+\pi/2) \\
%         \end{bmatrix}\\[0.5em]
%         &\theta^*_{obj} = \theta_{ref} - \theta_{obj} - \pi/2 
%     \end{aligned}
% \end{equation}




% In this equation, $\left[O_x,O_y\right]$ and $\left[O_{R_x},O_{R_y}\right]$ represent the objects and reflector center location in the original coordinate, and $\theta_{ref}$ represents the reflector orientation. "$^*$" sign represents the objects' properties in the reflector coordinate systems. Additionally, since we want to consider the reflection off of the reflector from both sides in \acrshort{design} we need to account for the proper modifications to simulate the reflection from the opposite side as well.
% \newline
% After, finding the EM wave propagation of the reflector plane now, we need to transform the calculated E-field to the original coordinate. In \acrshort{design}, we use the $\mathcal{R}^{-1}_r$ transformation matrix to find the converted grid and ultimately find the E-field in the original coordinates through linear interpolation in discretized grid points.
% \newline
%  \acrshort{design}'s core algorithm is summarized in \ref{algorithm}.  \acrshort{design} considers an arbitrary number of reflections using a user-defined parameter describing the depth of EM wave propagation. That is to say, in \acrshort{design} we have designed a recursive algorithm to consider the reflections off of the consecutive reflectors/RIS planes. \acrshort{design} algorithm implements the simulator design sections step-by-step in a recursive manner to accurately and efficiently compute the near-field channel. 



%RMSE is defined as follows:
% \begin{equation}
%     RMSE = \sqrt{\frac{1}{N^2}\sum_{i=1}^{N} \sum_{j=1}^{N} (|E_{s_{i,j}}| - |E_{f_{i,j}}|)^2}
%     \nonumber
% \end{equation}
%Where $|E_s|$ and $|E_f|$ represent $N\times N$ matrices of the E-field absolute value at N discrete locations in the environment obtained from the \acrshort{design} and Altair Feko simulators, respectively.

%\begin{equation}
%\begin{aligned}
%%    &\rho_{u,v} =\frac{1}{N^2} \sum_{i=1}^{N} \sum_{j=1}^{N} %\frac{\sigma_{|E_f||E_s|}}{\sigma_{|E_f|} \sigma_{|E_s|}}\\
%    &\sigma_{|E_f||E_s|} = (|E_{f_{(i,j)}}| - \mu_{|E_f|})\left(|E_{s_{((i+u),(j+v))}}| - \mu_{|E_s|})\right)
%\end{aligned}
%\nonumber
%\end{equation}


\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/0.1_rough.eps}
        \caption{Feko ($0.1mm$)}
        \label{fig:feko_rough_1}
    \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/0.3_rough.eps}
        \caption{Feko ($0.3mm$)}
        \label{fig:feko_rough_3}
    \end{subfigure}
        \centering
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/0.5_rough.eps}
        \caption{Feko ($0.5mm$)}
        \label{fig:feko_rough_5}
    \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/0.6_rough.eps}
        \caption{Feko ($0.6mm$)}
        \label{fig:feko_rough_6}
    \end{subfigure}
        \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/0.9_rough.eps}
        \caption{Feko ($0.9mm$)}
        \label{fig:feko_rough_9}
    \end{subfigure}
        \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/0.1_rough_sim.eps}
        \caption{\acrshort{design} ($0.1mm$)}
        \label{fig:sim_rough_1}
    \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/0.3_rough_sim.eps}
        \caption{\acrshort{design} ($0.3mm$)}
        \label{fig:sim_rough_3}
    \end{subfigure}
        \centering
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/0.5_rough_sim.eps}
        \caption{\acrshort{design} ($0.5mm$)}
        \label{fig:sim_rough_5}
    \end{subfigure}
    \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/0.6_rough_sim.eps}
        \caption{\acrshort{design} ($0.6mm$)}
        \label{fig:sim_rough_6}
    \end{subfigure}
        \begin{subfigure}[b]{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/0.9_rough_sim.eps}
        \caption{\acrshort{design} ($0.9mm$)}
        \label{fig:sim_rough_9}
    \end{subfigure}
    \caption{Samples of diffuse rough scattering simulations in \acrshort{design} and Feko for fixed $L_c=3mm$ and different $h_{rms}$ values.}
    \label{fig:rough_samples}
\end{figure*}


\subsubsection{Non-Scapular Reflection with RIS}
To assess the performance of the \acrshort{design} in simulating RIS with specific phase configurations, we simulate 10 different RIS configurations \yg{is it near-field} such that it redirects an incident beam with the incident angle of \yg{x} to different non-specular angles ranging from \yg{x} to \yg{y}. The phase profile on RIS to create such non-specular reflection is calculated by the user through a straightforward theoretical derivation assuming a point source. Fig. \ref{fig:RIS_regular} demonstrates the observed reflected angle in \acrshort{design} vs the theoretical reflection angle. \yg{complete}

we first outline the theory behind designing RIS phase shifts to redirect the incident wave in a non-specular direction. Then, we compare the simulation results from a standard reflector plane and the designed RIS to see how well RIS redirects the incident wave to a desired angle. We assume a Tx antenna array with an E-field distribution that emits a Gaussian beam steering towards an angle $\theta_{steer}$. The RIS is positioned in the near-field region of the Tx antenna at $(O_x, O_y)$, oriented with $\theta_{RIS} = 0$, and has a length $R_L$. Consequently, the incident beam on the RIS plane can be described by $\theta_{steer} = \theta_{inc}$. To reflect the beam toward $\theta_{des}$, the required phase shifts for the RIS plane are calculated using the formula:
 \begin{equation}
     \phi_n = -k(r_n+x_n(sin(\theta_{des})-sin(\theta_{inc}))-\frac{x_n^2}{2R})
 \end{equation}
where $n$ denotes the \textit{$n^{th}$} RIS element, $R$ is the distance from the Tx antenna to the center of the RIS plane, $x_n$ is the position of the \textit{$n^{th}$} RIS element, and $r_n = \sqrt{R^2 + x_n^2}$. It should be noted that this formula is an approximation for point source antenna and does not guarantee a perfect non-specular reflection toward $\theta_{des}$ in near-field when there is a large TX aperture. However, it sufficiently demonstrates \acrshort{design}'s capability to simulate RIS.
\newline
We now simulate a sample scenario for non-specular reflection using RIS. With the previous conditions applied and $\theta_{inc} = 45^\circ$ and $\theta_{des} = 60^\circ$, Fig. \ref{fig:RIS_regular} shows the coverage maps resulting from both the regular reflection and the designed RIS. The results illustrate that the RIS plane effectively redirects the incident beam towards 60 degrees, while the regular reflector produces a specular reflection at 45 degrees.
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/regular.eps}
        \caption{Specular reflection}
        \label{fig:regular_ref}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/redirected.eps}
        \caption{RIS non-specular reflection}
        \label{fig:RIS}
    \end{subfigure}
    \caption{Comparison between standard reflection and RIS designed non-specular reflection.\yg{placeholder- will be updated with new figure}}
    \label{fig:RIS_regular}
\end{figure}


% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/airy_feko.pdf}
%         \caption{Feko}
%         \label{fig:Airy_feko}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/airy_sim.pdf}
%         \caption{\acrshort{design}}
%         \label{fig:Airy_sim}
%     \end{subfigure}
%     \caption{Airy beam simulation in \acrshort{design} and Feko.}
%     \label{fig:Airy}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/bessel_feko.pdf}
%         \caption{Feko}
%         \label{fig:Bessel_feko}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/bessel_sim.pdf}
%         \caption{\acrshort{design}}
%         \label{fig:Bessel_sim}
%     \end{subfigure}
%     \caption{Bessel beam simulation in \acrshort{design} and Feko.}
%     \label{fig:Bessel}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/focusing_feko.eps}
%         \caption{Feko}
%         \label{fig:focus_feko}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/focusing_sim.eps}
%         \caption{\acrshort{design}}
%         \label{fig:focus_sim}
%     \end{subfigure}
%     \caption{Beam focusing simulation in \acrshort{design} and Feko.}
%     \label{fig:focus}
% \end{figure}


% \begin{figure*}
    
% \end{figure*}

 %In traditional wireless networks operating at microwave and lower millimeter-wave frequencies (such as Wi-Fi, LTE, and 5G), nodes typically operate in the far-field region of transmitting antennas~\cite{liu2023near}. 
%For example, the near field of a 10 cm planar array at 3 GHz is only a few tens of centimeters, whereas the near field for the same antenna footprint at 300 GHz extends to a few tens of meters. 


%To achieve a more scalable solution, various statistical channel modeling frameworks have been developed for mm-waive communication systems. 3rd Generation Partnership Project (3GPP) \cite{} has been established to characterize the behavior of radio channels by capturing the statistical properties of the signal as it propagates through the environment. 3GPP develops its statistical channel models based on extensive practical measurements gathered through various experimental campaign in different environments, such as urban, suburban, rural, indoor, and vehicular scenarios, across a range of frequencies. The NYUSIM \cite{} channel simulation software, which can be used to generate realistic temporal and spatial mm-waive channel  responses is another example of statistical channel simulators developed based on practical measurements. While statistical channel modeling can be efficient for mm-wave far-field wireless systems, it fails to capture the site-specific near-field EM wave propagation behavior of large Tx antenna arrays with arbitrary phase configurations.

%On the other hand, several ray tracing methods have been presented to overcome the scalability challenges of EM simulators and provide accurate site-specific channel simulations. Sionna \cite{hoydis2022sionna} which is a GPU-accelerated open-source library developed for next-generation physical layer studies, integrates a differentiable ray tracer (RT) for the simulation of radio wave propagation in user-defined environments and can be scalable for various AI-enabled applications. However, ray tracing methods calculate the channel impulse response based on far-field assumptions and fail to capture the near-field characteristics. In Sionna RT \cite{10465179} one can determine the TX antenna patterns and array geometry, and then calculate the far field channel at different locations assuming the total electric field radiating pattern of the TX antenna arrays is spherical shaped with standard beam-forming gain patterns. However, in order to capture the near-field EM wave propagation characteristics accurately we should consider each of the TX antenna array elements radiating spherical waves. It should be noted that placing a large number of isotropic antenna elements with $\lambda/2$ spacing in ray tracing simulators is not scalable. Solving this configuration even in free space in the RT environment would take significantly longer ($20 \times$) as compared to solving the same configuration in intensive EM simulators like Feko \footnote{Ray tracing simulation takes around 15 minutes to run on T4 GPU while the same configuration takes around 30s in Feko running on CPU (18-core server)}. Consequently, ray tracing simulators would also fail to accurately capture near-field EM wave propagation behavior of large TX antenna arrays with arbitrary phase configuration. 
